Analytical Models for Particle Diffusion and Flow in a Horizontal Cylinder with a Vertical Force

This paper considers particle propagation in a cylindrical molecular communication channel, e.g. a simplified model of a blood vessel. Emitted particles are influenced by diffusion, flow, and a vertical force induced e.g. by gravity or magnetism. The dynamics of the diffusion process are modeled by multi-dimensional transfer functions in a spatio-temporal frequency domain. Realistic boundary conditions are incorporated by the design of a feedback loop. The result is a discrete-time semi-analytical model for the particle concentration in the channel. The model is validated by comparison to particle-based simulations. These numerical experiments reveal that the particle concentration of the proposed semi-analytical model and the particle-based model are in excellent agreement. The analytical form of the proposed solution provides several benefits over purely numerical models, e.g. high flexibility, existence of low run-time algorithms, extendability to several kinds of boundary conditions, and analytical connection to parameters from communication theory.

==> analysis.tex <==
\vspace*{-2ex}
\section{Analysis and Evaluation}
\label{sec:analysis}

This section analyzes the proposed algorithm for the semi-analytical model in view of runtime and accuracy. Also, the benefits of a semi-analytical model over pure numerical models are discussed. 
\vspace*{-1.5ex}
\subsection{Algorithm Analysis}
\label{subsec:ana}
%In this section the proposed algorithm is analyzed with respect to runtime, accuracy and complexity. Especially the trade-off between runtime and accuracy is discussed. 
%
Fig.~\ref{fig:4} shows two plots of the concentration $p_{\mathrm{r},z = 75}(\bm{x}_1,t)$ in the receiver simulated with the proposed model \eqref{eq:35} at the bottom of the cylinder. 
The left plot follows the blue line in Fig.~\ref{fig:6}, the signal at $z = 75$ with a drift velocity of $u=3$. 
%
The simulations are done for a decreasing number of terms $Q = N\cdot M$ (compare \eqref{eq:9}). The order range $n$ of the Bessel functions is fixed to $N = 41$ and the range of $\mu$ is varied $M = 70, 20, 10, 5$. The empty dots are the result of the particle based simulation as ground truth. 
%
The right plot in Fig.~\ref{fig:4} shows the receiver concentration $p_\mathrm{r}$ at time $t = 0.15$ as a function of $u$ for decreasing number of terms. 
%
As already shown in Section~\ref{subsec:cs} for $N=41, M =70$ the particle simulation and the results of the proposed semi-analytical model match perfectly. 

The runtime is $t_{2870} = 125\,\si{s}$ to simulate a normalized duration of  $t_\mathrm{dur} = 0.5$ starting at $t = 0$.
%
For $Q = 820$ the semi-analytical model still matches the results of the particle model nearly perfectly, the runtime decreases to $t_{820} = 4.5\,\si{s}$. 
%
A further reduction of the number of terms leads to visible deviations, but the runtime drops to $t_{410} = 0.9\,\si{s}$, $t_{210} = 0.5\,\si{s}$. For comparison, the runtime of the particle based simulation is approx. $t_\mathrm{p} \approx 30\,\si{min}$ to simulate $0.5$ normalized time-units. 
%
The results in Fig.~\ref{fig:6} reveal a trade-off between runtime and accuracy. This shows the flexibility of the proposed model, depending on the purpose of an experiment: To simulate exact concentrations the number of terms, $Q$, can be increased at the cost of runtime. To study the rough behavior of a channel due to parameter variations, the number of terms can be reduced to run several simulations in a short time.
%
The right hand side plot in Fig.~\ref{fig:4} reveals that the accuracy also depends on the velocity $u$ and decreases for increasing $u$. 
%For an analysis of the complexity of the algorithm, the most interesting step is the iteration over time in step 7 (table~\ref{tab:1}), which depends on the programming language. Using a representation of \eqref{eq:33} in terms of sums \eqref{eq:9} leads to a nesting of three \texttt{for}-loops, which leads to a complexity of $\mathcal{O}(n^3)$. Using a vector-based implementation of \eqref{eq:33} reduces the number of \texttt{for}-loops and results in a complexity of $\mathcal{O}(n)$.


\begin{figure}
	\begin{minipage}{0.45\linewidth}
		\hspace*{-5ex}
%		\input{./../Bilder/uCompare.tex}
 \includegraphics{termCompare}
	\end{minipage}\hfill
	\begin{minipage}{0.45\linewidth}
		\hspace*{-5ex}
%		\input{./../Bilder/termCompare2.tex}
  \includegraphics{uCompare}
	\end{minipage}
	\vspace*{-3ex}
	\caption{\small Receiver concentration $p_{\mathrm{r},z=75}(\bm{x}_1,t)$ over time (left) and for increasing $u$ at $t = 0.15$ (right) with the proposed model for decreasing number of terms $Q=2870, 820, 410, 205$.}
	\label{fig:4}
	\vspace*{-4.5ex}
\end{figure}

\vspace*{-1.8ex}
\subsection{Benefits of the Semi-Analytical Model}

The proposed semi-analytical model in state-space description (see Section~\ref{sec:model}) offers many advantages over purely numerical models. 

The semi-analytical description of the diffusion process allows to compute the channel impulse response in an analytical manner.
Solutions in the form of \eqref{eq:32} can be related to parameters relevant for communications system design (e.g. inter-symbol interference) more easily than solutions with pure numerical models. Additionally, the complexity of the simulation algorithm is flexible (vary $M,N$), to focus the simulation on single relevant parameters. Knowing the eigenvalues $s_{\mu,n}$ of the diffusion process provides insight into the behavior of the process, e.g. damping or asymptotic behavior. As the output variable $\bm{y}$ in \eqref{eq:32} also contains the fluxes $\bm{i}$, they can be simulated without any additional effort.

The formulation of the solution in terms of a state-space description in Section \ref{subsubsec:ssd} with the general boundary term $\bar{\bm{\Phi}}(s)$ can be extended to different kinds of boundary conditions. In this paper, the techniques from Section~\ref{subsec:fcl} are used to realize the boundary conditions \eqref{eq:p9}. By the same technique also other types of boundary behavior of interest can be realized, e.g. semi-permeable membranes or non-reflective cell walls \cite{lnt2017-47}. The incorporation of different boundary conditions can be interpreted as an extension of the general state-space description, so the computation of the general model (Steps 1-3 in Table \ref{tab:1}) stays the same. This allows the simulation of complex diffusive systems/channels in a semi-analytical way by the separation of the general model from the desired boundary behavior. 

Also, the interconnection of several semi-analytical models for larger biochemical structures is possible by the techniques shown in Section~\ref{subsec:fcl} \cite{Willems:ICS:2007:4384643}. E.g. several cylindrical models can be used to model a structure of neighboring blood vessels, or several spherical models can realize complex interacting cell structures. 

==> introduction.tex <==
%Title: Magnetic Nanoparticles for Molecular Communication in Blood Vessels -- A Transfer Function Approach
\vspace*{-1.6ex}
\section{Introduction}

%Molecular communication in general
%The application of communications engineering to biotechnological devices by changing the mode of transmission from electromagnetic waves to the transport of molecules prompted a large interest, see \cite{Farsad_comprehensive_2016} for a review of the recent literature.
%Conventional communication techniques rely on the propagation of electromagnetic or acoustic waves. 
%
%The recent interest in biology-inspired communication has revealed the need to investigate the transport of molecules as carriers of information instead of electromagnetic or acoustic waves, see \cite{Farsad_comprehensive_2016} for a review of the recent literature.
%
The application of communications engineering principles to biotechnological problems has  prompted a large interest and has motivated the investigation of the transport of molecules as carriers of information, see \cite{Farsad_comprehensive_2016} for a review of recent literature.


%Active transport
The transport of molecules, or more generally particles, differs fundamentally from the propagation of electromagnetic waves and therefore requires new theoretical models for system design and analysis \cite{Farsad_comprehensive_2016}.
Though negligible at macroscale, the transport by diffusion becomes relevant at nanoscale.
However, diffusion can be slow and thus relying only on diffusion might be limited to small distances such as in intracellular communication.
In fact, in biotechnology, active transport mechanisms induced by an external force, fluid flow, or a combination thereof are well established \cite{Fournier_Basic_2017}.
%Magnetic nanoparticles
In particular, magnetic forces are attractive because the magnetization of biological particles is often negligible and special purpose magnetic nanoparticles can be engineered and tailored to an application by adapting their size and composition \cite{Pankhurst_Applications_2003}.
In this way, magnetic nanoparticles can be selectively detected and externally steered in a preferred direction by applying a magnetic field. % \cite{Pankhurst_Applications_2003}.
Furthermore, magnetic nanoparticles can be made biocompatible by a suitable coating which can avoid reactions with undesired reactants and allow for specific binding to others \cite{Pankhurst_Applications_2003}.

%Magnetic nanoparticles in molecular communication
%Inspired by their versatility in biotechnology, the use of magnetic nanoparticles for molecular communication was studied in \cite{Kisseleff_Magnetic_2017} and \cite{Wicke_Molecular_2017}.
%In particular, \cite{Kisseleff_Magnetic_2017} proposed a wearable device for detecting particles moving through a coil and \cite{Wicke_Molecular_2017} investigated the benefits of using magnetic nanoparticles as attractable information carriers in a two-dimensional flow system.
%Simplified models
%While the focus of \cite{Wicke_Molecular_2017} was in introducing the particles as information carriers, the considered system model was simplistic in considering a two-dimensional environment.
%
%However, investigating the particle transport in a blood vessel is of high interest for molecular communication due to its practicality \cite{Felicetti_Modeling_2014,Chahibi_molecular_2013,He_Channel_2016}.
Motivated by the concept of using magnetic nanoparticles for molecular communication proposed in \cite{Wicke_Molecular_2017} and the practicality of studying blood vessels \cite{Felicetti_Modeling_2014,Chahibi_molecular_2013,He_Channel_2016}, here we consider particle transport subject to horizontal fluid flow, diffusion, and a vertical magnetic force in a cylinder model of a blood vessel.
%Thereby, f in axial direction
For simplicity, we assume a uniform axial flow, which is a typical model known as plug flow \cite{Levenspiel_Chemical_1999}. Although blood vessels may have a complicated shape, modeling them as cylinders is well-accepted \cite{Fournier_Basic_2017}. To study the distribution of particles along a segment of the vessel wall, a line receiver model is considered.

When neglecting diffusion, the particle trajectory in a cylinder due to fluid flow and magnetic force can be accurately modeled even for more complicated flow patterns \cite{Furlani_analytical_2006}.
However, modeling diffusion, flow, and particle drift by magnetic force in a cylinder is analytically demanding due to the non-symmetry of the problem.
%Numerical simulation
Therefore, usually finite element numerical simulation is employed to study this type of system, e.g., in drug-targeting \cite{Nacev_behaviors_2011,Afkhami_Ferrofluids_2017}.
%This type of model is also useful for experiments \cite{Janikowska_novel_2017}.
%However, a numerical solution does not give insight into the transport process.
However, numerical solutions lead to algorithms with typically long run-times and low flexibility due to changing channel parameters. 


%Our approach: semi-analytic model
%The semi-analytic form is much better than a purely numerical scheme...
A different modeling technique is the application of functional transformations, which are based on the modal expansion of an initial boundary value problem \cite{Curtain:1995:IIL:207416,churchill:1972}. The technique has been already applied successfully, e.g. in the field of sound synthesis and circuit modeling, see \cite{lnt2017-47,antonini2012} for further references. 
%
%
This kind of modeling technique offers several benefits: It leads to semi-analytical models in terms of a state-space description which provide insights into the diffusion process.
%from an engineering point of view
Furthermore, these models allow the adaption of their boundary behavior using feedback techniques \cite{lnt2017-47,Willems:ICS:2007:4384643,Deutscher:IJC:2009}.
%Applicability


%Our contribution
%The proposed framework is extensible to different boundary conditions and ...
%The used algorithm is fast ...
%In this paper, a semi-analytical model for the diffusion process in a cylinder with a vertical magnetic force is derived in terms of a state space description.   

This paper proposes a semi-analytical model for a diffusive cylindrical molecular communication channel in the presence of a magnetic force and flow. The model leads to a low run-time simulation algorithm, which provides several benefits compared to purely numerical models.  
%
%This leads to a discrete-time simulation algorithm for the spatial concentration of particles in a receiver.
%The derived model can also serve as a blueprint for scenarios with different boundary conditions. 
Our results might be useful for scenarios studying, e.g. blood vessels, flow reactors or microfluidics. It could also be interesting for the study of diffusion with horizontal slurry flow in tubes where particles sediment due to gravity \cite[Chapter~13]{brennen2005fundamentals}.
%The validity of the model is shown by simulation and comparison with particle-based simulation results. 

%Paper structure
The paper is structured as follows: In Section~\ref{sec:prob}, a physical description of the scenario under study is presented.
%in terms of an initial-boundary-value problem
%, which is then formulated in a unifying vector form
In Section~\ref{sec:model}, a semi-analytical model for the diffusive cylindrical channel is derived and a simulation algorithm is proposed. The validity of the model is shown in Section~\ref{sec:experiments} by simulation, and the algorithm is analyzed and its benefits are discussed. Finally, Section~\ref{sec:conclusion} concludes the paper and proposes topics for further work.  
%Magnetic nanoparticles in molecular communication

%Numerical simulation studies

%Plug flow reactor model

%Beschreibung Szenario und fr\"uhere Arbeiten:
%\begin{itemize}
%	\item Molekulare Kommunikation unter Zuhilfenahme von magnetischen Nanopartikeln
%	\item Blutgef\"{a}\ss e und Approximation durch Zylinder; Modelle und fr\"uhere Arbeiten in der Literatur
%\end{itemize}
%
%Beschreibung der Methode: 
%\begin{itemize}
%	\item Modale Zerlegung als sinnvolle Methode zur Bildung von semi-analytischen Modellen
%	\item Konzepte aus der Regelungstechnik zur Einbindung komplexer Randbedingungen 
%\end{itemize}
%
%Beschreibung der Arbeiten im Paper 
%\begin{itemize}
%	\item Was wird hier untersucht 
%	\item Beschreibung des Beitrags und weitere Möglichkeiten der Anwendung (drug targeting, Schwerkraft, Petrischale)
%	\item Paper Struktur
%\end{itemize}


==> tikzlibrarydsp.code.tex <==
% -------------------------------------------------------------------------
% This library for block diagrams and signal flow graphs was inspired by
% the library "signalflow" of Dr. Karlheinz Ochs, Ruhr-University of Bochum,
% Germany. Furthermore, some ideas were taken from the library "circuitikz"
% of Massimo A. Redaelli and from the PGF library itself.
%
% Copyright 2012 by Matthias Hotz
%
% This work is licensed under the Creative Commons Attribution 2.5 Generic
% License. To view a copy of this license, visit
%          http://creativecommons.org/licenses/by/2.5/
% or send a letter to Creative Commons, 444 Castro Street, Suite 900,
% Mountain View, California, 94041, USA.
% -------------------------------------------------------------------------

\usetikzlibrary{arrows, calc, positioning, decorations.markings}

% -------------------------------------------------------------------------
% Parameters for the library

\newcommand{\dsplinewidth}{0.25mm}           % Line width for connections
\newcommand{\dspblocklinewidth}{0.3mm}       % Line width for blocks
\newcommand{\dspoperatordiameter}{4mm}       % Diameter for adder, multiplier, mixer
\newcommand{\dspoperatorlabelspacing}{2mm}   % Distance from symbol to label for adder, multiplier, mixer
\newcommand{\dspnoderadius}{1mm}             % Filled and empty node
\newcommand{\dspsquareblocksize}{8mm}        % Size for square blocks, e.g. for delay elements, decimator, expander
\newcommand{\dspfilterwidth}{14mm}           % Width of a filter block

% -------------------------------------------------------------------------
% Define new arrow heads

\pgfarrowsdeclare{dsparrow}{dsparrow}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfarrowsleftextend{-4\arrowsize}
	\pgfarrowsrightextend{4\arrowsize}
}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfsetdash{}{0pt} % Solid line (do not dash)
	\pgfsetmiterjoin	 % Fixed miter join of line
	\pgfsetbuttcap		 % Fixed butt cap of line
	\pgfpathmoveto{\pgfpoint{-4\arrowsize}{2.5\arrowsize}}
	\pgfpathlineto{\pgfpoint{4\arrowsize}{0pt}}
	\pgfpathlineto{\pgfpoint{-4\arrowsize}{-2.5\arrowsize}}
	\pgfpathclose
	\pgfusepathqfill
}

\pgfarrowsdeclare{dsparrowmid}{dsparrowmid}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfarrowsleftextend{-4\arrowsize}
	\pgfarrowsrightextend{4\arrowsize}
}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfsetdash{}{0pt}
	\pgfsetmiterjoin
	\pgfsetbuttcap
	\pgfpathmoveto{\pgfpoint{0}{2.5\arrowsize}}
	\pgfpathlineto{\pgfpoint{8\arrowsize}{0pt}}
	\pgfpathlineto{\pgfpoint{0}{-2.5\arrowsize}}
	\pgfpathclose
	\pgfusepathqfill
}

% -------------------------------------------------------------------------
% Define new node shapes

\makeatletter

\pgfkeys{/tikz/dsp/label/.initial=above}

% Generic shape generator for operators, i.e. nodes with a circular
% shape with an additional customizable drawing and a text label
\long\def\dspdeclareoperator#1#2{
	\pgfdeclareshape{#1}
	{
		% Saved anchors, macros and dimensions
		\savedanchor\centerpoint{\pgfpointorigin}
		\savedmacro\label{\def\label{\pgfkeysvalueof{/tikz/dsp/label}}}
	  \saveddimen\radius
	  {
		  \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
		  \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
	    \ifdim\pgf@xa>\pgf@ya
	      \pgf@x=.5\pgf@xa
	    \else
	      \pgf@x=.5\pgf@ya
	    \fi
	  }
	  
	  % Inherit all anchors from the 'circle'-shape:
	  \inheritanchor[from={circle}]{center}
	  \inheritanchor[from={circle}]{mid}
	  \inheritanchor[from={circle}]{base}
	  \inheritanchor[from={circle}]{north}
	  \inheritanchor[from={circle}]{south}
	  \inheritanchor[from={circle}]{west}
	  \inheritanchor[from={circle}]{east}
	  \inheritanchor[from={circle}]{mid west}
	  \inheritanchor[from={circle}]{mid east}
	  \inheritanchor[from={circle}]{base west}
	  \inheritanchor[from={circle}]{base east}
	  \inheritanchor[from={circle}]{north west}
	  \inheritanchor[from={circle}]{south west}
	  \inheritanchor[from={circle}]{north east}
	  \inheritanchor[from={circle}]{south east}
	  \inheritanchorborder[from={circle}]
	  
	  % Draw circle and embed additional code
	  \backgroundpath
	  {
	    % Draw circle
	    \pgfpathcircle{\centerpoint}{\radius}
	    
	    % Embed additional code
	    % (Note that this code must call e.g. \pgfusepathqstroke
	    #2
	  }
	
		% Define anchor parametrized by the PGF key /tikz/dsp/label
	  \anchor{text}
	  {
			\centerpoint
			%
	    \def\templabelabove{above}
	    \def\templabelbelow{below}
	    \def\templabelleft{left}
	    \def\templabelright{right}
	    \pgfutil@tempdima=\dspoperatorlabelspacing
	    %
	    \ifx\label\templabelabove
				\advance\pgf@x by -0.5\wd\pgfnodeparttextbox
				\advance\pgf@y by \radius
				\advance\pgf@y by \pgfutil@tempdima
	    \fi
	    %
	    \ifx\label\templabelbelow
				\advance\pgf@x by -0.5\wd\pgfnodeparttextbox
				\advance\pgf@y by -\radius
				\advance\pgf@y by -\pgfutil@tempdima
				\advance\pgf@y by -\ht\pgfnodeparttextbox
	    \fi
	    %
	    \ifx\label\templabelleft
				\advance\pgf@x by -\radius
				\advance\pgf@x by -\pgfutil@tempdima
				\advance\pgf@x by -\wd\pgfnodeparttextbox
				\advance\pgf@y by -0.5\ht\pgfnodeparttextbox
				\advance\pgf@y by +0.5\dp\pgfnodeparttextbox
	    \fi
	    %
	    \ifx\label\templabelright
				\advance\pgf@x by \radius
				\advance\pgf@x by \pgfutil@tempdima
				\advance\pgf@y by -0.5\ht\pgfnodeparttextbox
				\advance\pgf@y by +0.5\dp\pgfnodeparttextbox
	    \fi
	  }
	}
}

\dspdeclareoperator{dspshapecircle}{\pgfusepathqstroke}

\dspdeclareoperator{dspshapecirclefull}{\pgfusepathqfillstroke}

\dspdeclareoperator{dspshapeadder}{
	% Coordinate offset for the plus
	\pgfutil@tempdima=\radius
	\pgfutil@tempdima=0.55\pgfutil@tempdima
	
	% Draw plus
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{0pt}{-\pgfutil@tempdima}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{0pt}{ \pgfutil@tempdima}}}
	
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{0pt}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{0pt}}}
	
	\pgfusepathqstroke
}

\dspdeclareoperator{dspshapemixer}{
	% Coordinate offset for the cross
	\pgfutil@tempdima=\radius
	\pgfutil@tempdima=0.707106781\pgfutil@tempdima
	
	% Draw cross
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{-\pgfutil@tempdima}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{ \pgfutil@tempdima}}}
	
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{ \pgfutil@tempdima}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{-\pgfutil@tempdima}}}
	
	\pgfusepathqstroke
}

\makeatother

% -------------------------------------------------------------------------
% Define node styles

\tikzset{dspadder/.style={shape=dspshapeadder,line cap=rect,line join=rect,
	line width=\dspblocklinewidth,minimum size=\dspoperatordiameter}}
\tikzset{dspmultiplier/.style={shape=dspshapecircle,line cap=rect,line join=rect,
	line width=\dspblocklinewidth,minimum size=\dspoperatordiameter}}
\tikzset{dspmixer/.style={shape=dspshapemixer,line cap=rect,line join=rect,
	line width=\dspblocklinewidth,minimum size=\dspoperatordiameter}}

\tikzset{dspnodeopen/.style={shape=dspshapecircle,line width=\dsplinewidth,minimum size=\dspnoderadius}}
\tikzset{dspnodefull/.style={shape=dspshapecirclefull,line width=\dsplinewidth,fill,minimum size=\dspnoderadius}}

% The fixed specification of text height and text depth is the somewhat
% unaesthetic workaround to align the text in different node at the same
% baseline. See the PGF/TikZ manual, ch. 5.1.
\tikzset{dspsquare/.style={shape=rectangle,draw,align=center,text depth=0.3em,text height=1em,inner sep=0pt,
	line cap=round,line join=round,line width=\dsplinewidth,minimum size=\dspsquareblocksize}}
\tikzset{dspfilter/.style={shape=rectangle,draw,align=center,text depth=0.3em,text height=1em,inner sep=0pt,
	line cap=round,line join=round,line width=\dsplinewidth,minimum height=\dspsquareblocksize,minimum width=\dspfilterwidth}}

% -------------------------------------------------------------------------
% Define "signal flow" lines

\tikzset{dspline/.style={line width=\dsplinewidth},line cap=round,line join=round}
\tikzset{dspconn/.style={->,>=dsparrow,line width=\dsplinewidth},line cap=round,line join=round}%line cap=rect,line join=miter}
\tikzset{dspflow/.style={line width=\dsplinewidth,line cap=round,line join=round,
  decoration={markings,mark=at position 0.5 with {\arrow{dsparrowmid}}},postaction={decorate}}}

% -------------------------------------------------------------------------
% Define various utility macros

\newcommand{\downsamplertext}[1]{\raisebox{0.1em}{$\big\downarrow$}#1}
\newcommand{\upsamplertext}[1]{\raisebox{0.1em}{$\big\uparrow$}#1}

